Hiding Behind Machines: When Blame Is Shifted to Artificial Agents

The transfer of tasks with sometimes far-reaching moral implications to autonomous systems raises a number of ethical questions. In addition to fundamental questions about the moral agency of these systems, behavioral issues arise. This article focuses on the responsibility of agents who decide on our behalf. We investigate the empirically accessible question of whether the production of moral outcomes by an agent is systematically judged differently when the agent is artificial and not human. The results of a laboratory experiment suggest that decision-makers can actually rid themselves of guilt more easily by delegating to machines than by delegating to other people. Our results imply that the availability of artificial agents could provide stronger incentives for decision makers to delegate morally sensitive decisions.

==> Discussion.tex <==
\section{Discussion}

Our results indicate that it is easier to predict a delegation decision based on principals self-percieved capabilities if agents are not human. This might be suprising to some. A significant amount of literature suggests that the use of technical aids is often biased and affected by an irrational aversion towards machine use (Parasuraman, 1997). Based on our findings however, we theorize, that non-human agents can have a rationalising effect on principals, especially in the moral domain. This can be explained by principals desire to delegate more than tasks or decisions themselves. They might be striving for psychological gains which can only be realized with the help of human agents. If the agents are non-human this aspect of the decision making process is taking a back seat to utility maximaziation. While further empirical research is needed to solidify this theory it could largely improve our understanding of human-machine-interaction in the moral domain.


==> Hypotheses.tex <==
\section{Background and Hypotheses}

Blaming problems on machines might be a common phenomenon but it is unclear whether people actually manage to exculpate themselves by doing so. We investigate wether people judge delegations to human and non-human agents differently to shed some light on this question. To achieve this, we will test the following hypothesis in a labortatory experiment.
\\ 
\\ 
\textbf{Hypothesis:} Delegators are rewarded/punished differently for delegating other-regarding tasks to machines as compared to humans.


Our hypothesis is based on the idea that people judge delegators differently if they give other-regarding tasks to machines instead of humans. The delegation of a task which could carry severe consequences for a third party to an unmonitored machine might result in punishment or defamation because the principal is considered careless. On the other hand principals might be exculpated entirely since people deem the failure of machines as being outside of their control. Either way, a better understanding of public reservations regarding the introduction of novel technology is likely to prove useful in future moral and legal considerations. The experiment designed to test the above hypothesis will be outlined in the following chapter.

Additionally we explored wether the effect of percieved utitlity on delegtion decisions varied depending on the nature of the agent. Based on a definition by \cite{dzindolet2002perceived} we define the perceived utility of employing a non-human agent as the difference between the perceived reliability of an automated device and the perceived reliability of manual control. We did also elicit the subjects attitudes towards risk. While both factors have not been our main focus, percieved utility and risk aversion are prominent in several ecoonmic applications including principal agent models \citep{o2018modeling}. We therefore included them to use it as a moderator in later analysis.

==> myreg_lin.tex <==
\begin{table}
\begin{center}
\begin{tabular}{lclc}
\toprule
\textbf{Dep. Variable:}    & Self-Assessment  & \textbf{  R-squared:         } &     0.302   \\
\textbf{Model:}            &       OLS        & \textbf{  Adj. R-squared:    } &     0.288   \\
\textbf{Method:}           &  Least Squares   & \textbf{  F-statistic:       } &     20.94   \\
\textbf{No. Observations:} &         149      & \textbf{            } &        \\
\bottomrule
\end{tabular}
\begin{tabular}{lcccccc}
                       & \textbf{coef} & \textbf{std err} & \textbf{t} & \textbf{P$>$$|$t$|$} & \textbf{[0.025} & \textbf{0.975]}  \\
\midrule
\textbf{Intercept}     &       3.5730  &        0.359     &     9.959  &         0.000        &        2.864    &        4.282     \\
\textbf{Error}         &       0.2507  &        0.079     &     3.185  &         0.002        &        0.095    &        0.406     \\
\textbf{Machine}       &      -0.8278  &        0.553     &    -1.497  &         0.136        &       -1.921    &        0.265     \\
\textbf{Error:Machine} &       0.3104  &        0.115     &     2.706  &         0.008        &        0.084    &        0.537     \\
\bottomrule

\end{tabular}

\caption{OLS Regression Results}
\label{tab:reglin}
\end{center}
\end{table}

